Comparison of HDR quality metrics in Per-Clip Lagrangian multiplier optimisation with AV1

The complexity of modern codecs along with the increased need of delivering high-quality videos at low bitrates has reinforced the idea of a per-clip tailoring of parameters for optimised rate-distortion performance. While the objective quality metrics used for Standard Dynamic Range (SDR) videos have been well studied, the transitioning of consumer displays to support High Dynamic Range (HDR) videos, poses a new challenge to rate-distortion optimisation. In this paper, we review the popular HDR metrics DeltaE100 (DE100), PSNRL100, wPSNR, and HDR-VQM. We measure the impact of employing these metrics in per-clip direct search optimisation of the rate-distortion Lagrange multiplier in AV1. We report, on 35 HDR videos, average Bjontegaard Delta Rate (BD-Rate) gains of 4.675%, 2.226%, and 7.253% in terms of DE100, PSNRL100, and HDR-VQM. We also show that the inclusion of chroma in the quality metrics has a significant impact on optimisation, which can only be partially addressed by the use of chroma offsets.

==> ieeedef.tex <==
\author{\IEEEauthorblockN{Vibhoothi}
\IEEEauthorblockA{\textit{Sigmedia Group, \\
Department of Electronic and Electrical Engineering, \\
Trinity College Dublin, Ireland. \\
vibhoothi@tcd.ie}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}




%% WORKING ONE

\author{\IEEEauthorblockN{Vibhoothi, Angeliki Katsenou, François Pitié, Anil Kokaram}
\IEEEauthorblockA{Sigmedia Group,\\
\textit{Department of Electronic and Electrical Engineering},\\
\textit{Trinity College Dublin},\\
Dublin, Ireland \\
\{vibhoothi, akatsenou, pitief, anil.kokaram\}@tcd.ie}
\and
\IEEEauthorblockN{Yeping Su, Balu Adsumilli}
\IEEEauthorblockA{Youtube Media-Algorithms Team,\\
\textit{Google Inc},\\
California, USA
\{yeping,badsumilli\}@google.com}
}



%% Full 6 authors
\author{\IEEEauthorblockN{Vibhoothi}
\IEEEauthorblockA{Sigmedia Group,\\
%\textit{Department of Electronic and Electrical Engineering},\\
\textit{Trinity College Dublin},\\
Dublin, Ireland \\
\{vibhoothi\}@tcd.ie}
\and
\IEEEauthorblockN{Angeliki Katsenou}
\IEEEauthorblockA{Sigmedia Group,\\
%\textit{Department of Electronic and Electrical Engineering},\\
\textit{Trinity College Dublin},\\
Dublin, Ireland \\
\{akatsenou\}@tcd.ie}
\and
\IEEEauthorblockN{François Pitié}
\IEEEauthorblockA{Sigmedia Group,\\
%\textit{Department of Electronic and Electrical Engineering},\\
\textit{Trinity College Dublin},\\
Dublin, Ireland \\
\{pitief\}@tcd.ie}
\and
\IEEEauthorblockN{Yeping Su}
\IEEEauthorblockA{
Youtube Media-Algorithms Team,\\
\textit{Google Inc},\\
California, USA \\
\{yeping\}@google.com}
\and
\IEEEauthorblockN{Balu Adsumilli}
\IEEEauthorblockA{
Youtube Media-Algorithms Team,\\
\textit{Google Inc},\\
California, USA \\
\{badsumilli\}@google.com}
\and
\IEEEauthorblockN{Anil Kokaram}
\IEEEauthorblockA{Sigmedia Group,\\
%\textit{Department of Electronic and Electrical Engineering},\\
\textit{Trinity College Dublin},\\
Dublin, Ireland \\
\{anil.kokaram\}@tcd.ie}
}

